Semantic Masking and Visual Feature Matching for Robust Localization

We are interested in long-term deployments of autonomous robots to aid astronauts with maintenance and monitoring operations in settings such as the International Space Station. Unfortunately, such environments tend to be highly dynamic and unstructured, and their frequent reconfiguration poses a challenge for robust long-term localization of robots. Many state-of-the-art visual feature-based localization algorithms are not robust towards spatial scene changes, and SLAM algorithms, while promising, cannot run within the low-compute budget available to space robots. To address this gap, we present a computationally efficient semantic masking approach for visual feature matching that improves the accuracy and robustness of visual localization systems during long-term deployment in changing environments. Our method introduces a lightweight check that enforces matches to be within long-term static objects and have consistent semantic classes. We evaluate this approach using both map-based relocalization and relative pose estimation and show that it improves Absolute Trajectory Error (ATE) and correct match ratios on the publicly available Astrobee dataset. While this approach was originally developed for microgravity robotic freeflyers, it can be applied to any visual feature matching pipeline to improve robustness.

==> degenerate_cases.tex <==
\begin{figure*}
    \centering

    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{images/superglue_degenerate_cases/13.jpg}
        \caption{Query Image}
        \label{fig:degenerate_motion_query_img}
    \end{subfigure}
    % \hspace{0.001\textwidth}  % Add some horizontal space between subfigures
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{images/superglue_degenerate_cases/13_map_image.jpg}
        \caption{Map Image}
        \label{fig:degenerate_motion_map_img}
    \end{subfigure}
    \begin{subfigure}[b]{0.5\textwidth}
        \includegraphics[width=\textwidth]{images/superglue_degenerate_cases/superglue_degenerate_motion.png}
        \caption{Matches after Semantic Post-Processing}
        \label{fig:degenerate_motion_matches}
    \end{subfigure}

    \caption{Degenerate Motion (rotation only, no translation)}
    \label{fig:degenerate_motion}
\end{figure*}
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{images/superglue_degenerate_cases/126.jpg}
        \caption{Query Image}
        \label{fig:degenerate_planar_query_img}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{images/superglue_degenerate_cases/126_map_img.jpg}
        \caption{Map Image}
        \label{fig:degenerate_planar_map_img}
    \end{subfigure}
     \begin{subfigure}[b]{0.5\textwidth}
        \includegraphics[width=\textwidth]{images/superglue_degenerate_cases/superglue_degenerate_planar.png}
        \caption{Matches After Semantic Post-Processing}
        \label{fig:degenerate_planar_matches}
    \end{subfigure}
    \caption{Degenerate Planar Scene}
    \label{fig:degenerate_planar}
\end{figure*}

==> double_matching_figure.tex <==
\twocolumn[{
\maketitle
\begin{center}
    \captionsetup{type=figure}
    \includegraphics[width=.5\textwidth]{images/astrobee_pair.jpg}
    \captionof{figure}{Test caption}
\end{center}
}]

==> error_tables.tex <==
\todo[inline]{bold good results, fix formatting, round numbers}
\sisetup{round-mode=places,round-precision=4}
% \begin{table*}[t]
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{cc|ccc|cc|ccc}
%     \toprule

% Sequence&&tb\_roll&tb\_pitch&tb\_yaw&ff\_return\_journey\_forward&ff\_return\_journey\_left&iva\_kibo\_trans&iva\_kibo\_rot&iva\_kibo\_tag  \\
%       \midrule
%       Astroloc Relocalizer &max:&\cellcolor[gray]{.8}\num{0.015403}&\num{0.026673}&\num{1.350333}&\num{1.437444}&\num{1.043529}&\num{3.405037}&\num{1.005764}&\num{1.167855}\\
%                             &median:&\num{0.005671}&\num{0.007639}&\num{0.032541}&\num{1.022843}&\num{0.334358}&\num{0.015037}&\num{0.017173}&\num{0.093657} \\
%                             &RMSE:&\cellcolor[gray]{.8}\num{0.007647}&\num{0.00953}&\num{0.30133}&\num{0.978852}&\num{ 0.337499}&\num{0.42808}&\num{0.098748}&\num{0.229465} \\
%       \midrule
%       Semantic Relocalizer &max:&0.015633&0.013847&0.376626&1.326094& 1.066863&2.068955&2.277931&0.530592\\
%                             &median:&\cellcolor[gray]{.8}0.005492&0.006259&0.032697&1.021239&0.329946&0.01563&0.014688&0.102779\\
%                             &RMSE:& 0.00846&0.00735&0.057787&0.970929&0.332322&0.259888&0.173117&0.129597\\
%          \bottomrule
%     \end{tabular}
%     }
%     \caption{Evaluation Results of ATE (unit: m) on Astrobee Datasets}
%     \label{tab: ate_table}

% \end{table*}

\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cc|ccc|cc|ccc}
    \toprule
Sequence&&tb\_roll&tb\_pitch&tb\_yaw&ff\_return\_journey\_forward&ff\_return\_journey\_left&iva\_kibo\_trans&iva\_kibo\_rot&iva\_kibo\_tag  \\
      \midrule
      Astroloc Relocalizer &max:&0.001764&0.006773&3.141498&0.184153&0.190478&0.563893&0.357659&0.889333\\
                            &median:&0.00082&0.002643&0.029714&0.006386&0.029229&0.004334&0.008638&0.072258\\
                            &RMSE:&0.000883&0.003237&1.474307&0.014822&0.036205&0.076822&0.034576&0.179128\\
      \midrule
      Semantic Relocalizer &max:&0.002231&0.006228&3.069498&0.441073&0.204514&0.366709&0.637306&0.361835\\
                            &median:&0.000865&0.003175&0.029167&0.006457&0.027218&0.004954&0.00498&0.085769\\
                            &RMSE:&0.000961&0.003351&0.202956&0.021205&0.034287&0.046994&0.055242&0.09838\\
         \bottomrule
    \end{tabular}
    }
    \caption{Evaluation Results of ARE (unit: degrees) on Astrobee Datasets}
    \label{tab: are_table}
\end{table*}

\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|ccc|cc|ccc}
    \toprule
Sequence&tb\_roll&tb\_pitch&tb\_yaw&ff\_return\_journey\_forward&ff\_return\_journey\_left&iva\_kibo\_trans&iva\_kibo\_rot&iva\_kibo\_tag  \\
      \midrule
      Astroloc Relocalizer &1.0&1.0&0.7755102040816326&0.04332344213649852
&0.30123099203475745&0.4812734082397004&0.7859424920127795&0.48026315789473684\\
      % \midrule
      Semantic Relocalizer &1.0&1.0&0.9428571428571428&0.04332344213649852&0.30340333091962346&0.5440074906367042 &0.7103301384451545&0.5263157894736842\\
         \bottomrule
    \end{tabular}
    }
    \caption{Evaluation Results of Success Rate on Astrobee Datasets}
    \label{tab: success_rate_table}
\end{table*}




==> error_tables_transposed.tex <==
\sisetup{round-mode=places,round-precision=4}
\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{
\begin{tabular}{l|ll|ll|ll}
    \toprule
                             & max                  &                      & median               &                      & RMSE                 &                      \\
Sequence                     & Baseline  & Semantic  & Baseline  & Semantic  & Baseline  & Semantic  \\
\toprule
tb\_roll                     & \cellcolor[gray]{.8}\num{0.015403}       & \num{0.015633}       & \num{0.005671}       & \cellcolor[gray]{.8}\num{0.005492}       & \cellcolor[gray]{.8}\num{0.007647}       & \num{0.00846}        \\
tb\_pitch                    & \num{0.026673}       & \cellcolor[gray]{.8}\num{0.013847}       & \num{0.007639}       & \cellcolor[gray]{.8}\num{0.006259}       & \num{0.00953}        & \cellcolor[gray]{.8}\num{0.00735}        \\
tb\_yaw                      & \num{1.350333}       & \cellcolor[gray]{.8}\num{0.376626}       & \cellcolor[gray]{.8}\num{0.032541}       & \num{0.032697}       & \num{0.30133}        & \cellcolor[gray]{.8}\num{0.057787}       \\
\midrule
ff\_return\_journey\_forward & \num{1.437444}       & \cellcolor[gray]{.8}\num{1.326094}       & \num{1.022843}       & \cellcolor[gray]{.8}\num{1.021239}       & \num{0.978852}       & \cellcolor[gray]{.8}\num{0.970929}       \\
ff\_return\_journey\_left    & \cellcolor[gray]{.8}\num{1.043529}       & \num{1.066863}       & \num{0.334358}       & \cellcolor[gray]{.8}\num{0.329946}       & \num{0.337499}       & \cellcolor[gray]{.8}\num{0.332322}       \\
\midrule
iva\_kibo\_trans             & \num{3.405037}       & \cellcolor[gray]{.8}\num{2.068955}       & \cellcolor[gray]{.8}\num{0.015037}       & \num{0.01563}        & \num{0.42808}        & \cellcolor[gray]{.8}\num{0.259888}       \\
iva\_kibo\_rot               &\cellcolor[gray]{.8} \num{1.005764}       & \num{2.277931}       & \num{0.017173}       & \cellcolor[gray]{.8}\num{0.014688}       & \cellcolor[gray]{.8}\num{0.098748}       & \num{0.173117}       \\
iva\_kibo\_tag               & \num{1.167855}       & \cellcolor[gray]{.8}\num{0.530592}       & \cellcolor[gray]{.8}\num{0.093657}       & \num{0.102779}       & \num{0.229465}       & \cellcolor[gray]{.8}\num{0.129597}    \\
\bottomrule
\end{tabular}
    }
     \caption{Evaluation Results of ATE (unit: m) on Astrobee Datasets}
    \label{tab:ate_table}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{
\begin{tabular}{l|ll|ll|ll}
 \toprule
                             & max                  &                      & median               &                      & RMSE                 &                      \\
Sequence                     & Baseline  & Semantic  & Baseline  & Semantic  & Baseline  & Semantic  \\
\toprule
tb\_roll                     & \cellcolor[gray]{.8}\num{0.001764}       & \num{0.002231}       & \cellcolor[gray]{.8}\num{0.00082}        & \num{0.000865}       & \cellcolor[gray]{.8}\num{0.000883}       & \num{0.000961}       \\
tb\_pitch                    & \num{0.006773}       & \cellcolor[gray]{.8}\num{0.006228}       & \cellcolor[gray]{.8}\num{0.002643}       & \num{0.003175}       & \cellcolor[gray]{.8}\num{0.003237}       & \num{0.003351}       \\
tb\_yaw                      & \num{3.141498}       & \cellcolor[gray]{.8}\num{3.069498}       & \num{0.029714}       & \cellcolor[gray]{.8}\num{0.029167}       & \num{1.474307}       & \cellcolor[gray]{.8}\num{0.202956}       \\
\midrule
ff\_return\_journey\_forward & \cellcolor[gray]{.8}\num{0.184153}       & \num{0.441073}       & \cellcolor[gray]{.8}\num{0.006386}       & \num{0.006457}       & \cellcolor[gray]{.8}\num{0.014822}       & \num{0.021205}       \\
ff\_return\_journey\_left    & \cellcolor[gray]{.8}\num{0.190478}       & \num{0.204514}       & \num{0.029229}       & \cellcolor[gray]{.8}\num{0.027218}       & \num{0.036205}       & \cellcolor[gray]{.8}\num{0.034287}       \\
\midrule
iva\_kibo\_trans             & \num{0.563893}       & \cellcolor[gray]{.8}\num{0.366709}       & \cellcolor[gray]{.8}\num{0.004334}       & \num{0.004954}       & \num{0.076822}       & \cellcolor[gray]{.8}\num{0.046994}       \\
iva\_kibo\_rot               &\cellcolor[gray]{.8} \num{0.357659}       & \num{0.637306}       & \num{0.008638}       & \cellcolor[gray]{.8}\num{0.00498}        & \cellcolor[gray]{.8}\num{0.034576}       & \num{0.055242}       \\
iva\_kibo\_tag               & \num{0.889333}       & \cellcolor[gray]{.8}\num{0.361835}       & \cellcolor[gray]{.8}\num{0.072258}       & \num{0.085769}       & \num{0.179128}       & \cellcolor[gray]{.8}\num{0.09838}    \\    
\bottomrule
\end{tabular}
    }
     \caption{Evaluation Results of ARE (unit: degrees) on Astrobee Datasets}
    \label{tab: are_table}
\end{table*}

\todo[inline]{some of the differences in the table (in gray) are pretty negligible...does highlighting them take away from the others?}
\begin{table*}[t]
    \centering
     \resizebox{0.5\textwidth}{!}{
\begin{tabular}{l|ll}
 \toprule

Sequence                     & Baseline & Semantic \\
\toprule
tb\_roll                     & \num{1}              & \num{1}              \\
tb\_pitch                    & \num{1}              & \num{1}              \\
tb\_yaw                      & \num{0.7755}         & \cellcolor[gray]{.8}\num{0.9429}         \\
\midrule
ff\_return\_journey\_forward & \num{0.0433}         & \num{0.0433}         \\
ff\_return\_journey\_left    & \num{0.3012}         & \cellcolor[gray]{.8}\num{0.3034}         \\
\midrule
iva\_kibo\_trans             & \num{0.4813}         & \cellcolor[gray]{.8}\num{0.544}          \\
iva\_kibo\_rot               & \cellcolor[gray]{.8}\num{0.7859}         & \num{0.7103}         \\
iva\_kibo\_tag               & \num{0.4803}         & \cellcolor[gray]{.8}\num{0.5263}  \\
\bottomrule
\end{tabular}
}
 \caption{Evaluation Results of Success Rate on Astrobee Datasets}
\label{tab: success_rate_table}
\end{table*}


==> matching_figures.tex <==

% \begin{figure}[ht]
% \begin{subfigure}[b]
% {0.99\linewidth}
%     \centering   \includegraphics[width=0.99\textwidth]{images/flag_match.png} % fix size and formatting
%         \caption{Matches with no semantic segmentation.}
   
%     \label{fig:flag_match}
% \end{subfigure}
% \begin{subfigure}[ht]
% {0.99\linewidth}
%     \centering
%     \includegraphics[width=0.99\textwidth]{images/semantic_flag_match.png} % fix size and formatting
%   \caption{Matches with semantic segmentation. Bounding boxes depict the semantic class detected (purple for vents, blue for lights, and red for handrails).}
%     \label{fig:semantic_flag_match}
% \end{subfigure}
%    % \caption{Matches between a query image (left) and map image (right) taken several years apart and with several scene changes, including a rotated flag that is upside-down in the right image. With no semantic segmentation as shown in Fig. \ref{fig:flag_match}, the strongest features are detected in the rotated flag, and the data association is made upside-down with respect to the map. With semantic segmentation applied to the feature matches as shown in Fig. \ref{fig:semantic_flag_match}, the associations are made correctly between the detected lights and vents and the scene inconsistencies in the flag are ignored.}
% \end{figure}

==> matching_figures_double_col.tex <==
% \twocolumn[{%
% \renewcommand\twocolumn[1][]{#1}%
% \maketitle
% \begin{figure}
% \begin{subfigure}[b]
% {0.99\linewidth}
%     \centering   \includegraphics[width=0.99\textwidth]{images/flag_match.png} % fix size and formatting
%         \caption{Matches with no semantic segmentation.}
   
%     \label{fig:flag_match}
% \end{subfigure}
% \begin{subfigure}[b]
% {0.99\linewidth}
%     \centering
%     \includegraphics[width=0.99\textwidth]{images/semantic_flag_match.png} % fix size and formatting
%   \caption{Matches with semantic segmentation. Bounding boxes depict the semantic class detected (purple for vents, blue for lights, and red for handrails).}
%     \label{fig:semantic_flag_match}
% \end{subfigure}
%    \caption{Matches between a query image (left) and map image (right) taken several years apart and with several scene changes, including a rotated flag that is upside-down in the right image. With no semantic segmentation as shown in Fig. \ref{fig:flag_match}, the strongest features are detected in the rotated flag, and the data association is made upside-down with respect to the map. With semantic segmentation applied to the feature matches as shown in Fig. \ref{fig:semantic_flag_match}, the associations are made correctly between the detected lights and vents and the scene inconsistencies in the flag are ignored.}
% \end{figure}
% }]

==> matching_figures_double_test.tex <==
\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\maketitle
%\newfloat{test}{htbp}{loc}
\captionsetup[test]{labelsep=space}
\begin{center}
    \centering
    \includegraphics[width=.99\textwidth,height=5cm]{images/flag_match.png}
            \captionof{test}{(a) Matches with no semantic segmentation.}
               \label{fig:flag_match}
        \centering
    \includegraphics[width=.99\textwidth,height=5cm]{images/semantic_flag_match.png}
            % \captionof{test}{(b) Matches with semantic segmentation. Bounding boxes depict the semantic class detected (purple for vents, blue for lights, and red for handrails).}
             \label{fig:semantic_flag_match}
    \captionof{figure}{Matches between a query image (left) and map image (right) taken several years apart and with several scene changes, including a rotated flag that is upside-down in the right image. With no semantic segmentation as shown in Fig. 1a, the strongest features are detected in the rotated flag, and the data association is made upside-down with respect to the map. With semantic segmentation applied to the feature matches as shown in Fig. 1b, the associations are made correctly between the detected lights and vents and the scene inconsistencies in the flag are ignored.}
\end{center}%
}]

==> pipeline_pic.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.3\textwidth, height=.18\textwidth]{images/bounding_boxes.png}
    \label{fig:boxes_img}
    \includegraphics[width=0.35\textwidth, height=.20\textwidth]{images/masked_images.png}
    \label{fig:masked_imgs}
    \includegraphics[width=0.49\textwidth]{images/pipeline-crop.pdf} % fix size and formatting
    % \includegraphics[width=0.49\textwidth]{images.pdf}
    \caption{The semantic image matching pipeline adds semantic segmentation stages in blue to a visual feature matching pipeline in red to improve pose estimation accuracy. The pipeline detects semantic objects in each image and generates masked image-space regions for each detection as shown in Fig.~\ref{fig:boxes_img}. It then detects visual features in the masked regions and performs matching between features of the same class for each pair of images. Finally, the pipeline estimates the relative pose between the images using the resulting matches.}
    \label{fig:pipeline}
\end{figure} 

==> superglue_tables.tex <==
Sequence                &                      & tb\_roll   & tb\_pitch  & tb\_yaw   & ff\_return\_journey\_forward & ff\_return\_journey\_left & iva\_kibo\_trans & iva\_kibo\_rot & iva\_kibo\_tag \\
error t (deg):          & Baseline             & \num{32.56072} & \num{22.86025}  & \num{24.5179}  & \num{35.79393} & \num{35.78241} & \num{43.83755} & \num{39.78524} & \num{25.41495} \\
error t (deg):          & Pre-Processing       & \num{35.77997} & \num{39.91108}  & \num{42.2196}  & \num{38.50315} & \num{45.91112} & \num{46.10867} & \num{45.77426} & \num{59.04471} \\
error t (deg):          & Post-Processing      & \num{13.92052} & \num{13.23055}  & \num{14.07822} & \num{19.02857} & \num{28.89392} & \num{33.41859} & \num{42.56035} & \num{42.09871} \\
error R (deg):          & Baseline             & \num{4.140139} & \num{2.990863}  & \num{5.965214} & \num{3.084002} & \num{5.95915} & \num{21.4706} & \num{14.00608} & \num{12.49089} \\
error R (deg):          & Pre-Processing       & \num{3.53702} & \num{4.956284}  & \num{10.6487}  & \num{6.211718} & \num{6.912781} & \num{27.54666} & \num{22.156} & \num{67.48147} \\
error R (deg):          & Post-Processing      & \num{2.032448} & \num{1.955149}  & \num{3.952338} & \num{3.375606} & \num{8.312445} & \num{13.53962} & \num{17.47411} & \num{21.68465} \\
correct match ratio:    & Baseline             & \num{0.65451} & \num{0.726771}  & \num{0.520139} & \num{0.278964} & \num{0.305618} & \num{0.191862} & \num{0.09507} & \num{0.443206} \\
correct match ratio:    & Pre-Processing       & \num{0.812111} & \num{0.790862}  & \num{0.595147} & \num{0.37581} & \num{0.349949} & \num{0.270376} & \num{0.104719} & \num{0.305245} \\
correct match ratio:    & Post-Processing      & \num{0.688818} & \num{0.745443}  & \num{0.584439} & \num{0.323893} & \num{0.33982} & \num{0.21298} & \num{0.098898} & \num{0.425435} \\
success rate:           & Baseline             & \num{1} & \num{1}  & \num{1} & \num{0.748815} & \num{0.691304} & \num{0.327103} & \num{0.161702} & \num{0.134868} \\
success rate:           & Pre-Processing       & \num{0.435484} & \num{0.98103} & \num{0.915} & \num{0.63981} & \num{0.473913} & \num{0.224299} & \num{0.12766} & \num{0.036184} \\
success rate:           & Post-Proccessing     & \num{1} & \num{1}  & \num{1} & \num{0.748815} & \num{0.691304} & \num{0.327103} & \num{0.161702} & \num{0.134868} \\
\end{tabular}
\end{table}


==> superglue_tables_transpose.tex <==
\sisetup{round-mode=places,round-precision=4}
\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{tabular}{l|rrr|rrr}
            \toprule
            Sequence & error t (deg): & & & error R (deg): & & \\
            & Baseline & Pre-Processing & Post-Processing & Baseline & Pre-Processing & Post-Processing \\
            \toprule
            tb\_roll & \num{32.56072} & \num{35.77997} & \cellcolor[gray]{.8}\num{13.92052} & \num{4.140139} & \num{3.53702} & \cellcolor[gray]{.8}\num{2.032448} \\
            tb\_pitch & \num{22.86025} & \num{39.91108} & \cellcolor[gray]{.8}\num{13.23055} & \num{2.990863} & \num{4.956284} & \cellcolor[gray]{.8}\num{1.955149} \\
            tb\_yaw & \num{24.5179} & \num{42.2196} & \cellcolor[gray]{.8}\num{14.07822} & \num{5.965214} & \num{10.6487} & \cellcolor[gray]{.8}\num{3.952338} \\
            \midrule
            ff\_return\_journey\_forward & \num{35.79393} & \num{38.50315} & \cellcolor[gray]{.8}\num{19.02857} & \cellcolor[gray]{.8}\num{3.084002} & \num{6.211718} & \num{3.375606} \\
            ff\_return\_journey\_left & \num{35.78241} & \num{45.91112} & \cellcolor[gray]{.8}\num{28.89392} & \cellcolor[gray]{.8}\num{5.95915} & \num{6.912781} & \num{8.312445} \\
            \midrule
            iva\_kibo\_trans & \num{43.83755} & \num{46.10867} & \cellcolor[gray]{.8}\num{33.41859} & \num{21.4706} & \num{27.54666} & \cellcolor[gray]{.8}\num{13.53962} \\
            iva\_kibo\_rot & \cellcolor[gray]{.8}\num{39.78524} & \num{45.77426} & \num{42.56035} & \cellcolor[gray]{.8}\num{14.00608} & \num{22.156} & \num{17.47411} \\
            iva\_kibo\_tag & \cellcolor[gray]{.8}\num{25.41495} & \num{59.04471} & \num{42.09871} & \cellcolor[gray]{.8}\num{12.49089} & \num{67.48147} & \num{21.68465} \\
            \bottomrule
        \end{tabular}
    }
\end{table*}

\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{tabular}{l|lll|lll}
            \toprule
            Sequence & correct match ratio: & & & success rate: & & \\
            & Baseline & Pre-Processing & Post-Processing & Baseline & Pre-Processing & Post-Proccessing \\
            \toprule
            tb\_roll & \num{0.65451} & \cellcolor[gray]{.8}\num{0.812111} & \num{0.688818} & \num{1} & \num{0.435484} & \num{1} \\
            tb\_pitch & \num{0.726771} & \num{0.790862} & \num{0.745443} & \num{1} & \num{0.98103} & \num{1} \\
            tb\_yaw & \num{0.520139} & \cellcolor[gray]{.8}\num{0.595147} & \num{0.584439} & \num{1} & \num{0.915} & \num{1} \\
            \midrule
            ff\_return\_journey\_forward & \num{0.278964} & \cellcolor[gray]{.8}\num{0.37581} & \num{0.323893} & \num{0.748815} & \num{0.63981} & \num{0.748815} \\
            ff\_return\_journey\_left & \num{0.305618} & \cellcolor[gray]{.8}\num{0.349949} & \num{0.33982} & \num{0.691304} & \num{0.473913} & \num{0.691304} \\
            \midrule
            iva\_kibo\_trans & \num{0.191862} & \cellcolor[gray]{.8}\num{0.270376} & \num{0.21298} & \num{0.327103} & \num{0.224299} & \num{0.327103} \\
            iva\_kibo\_rot & \num{0.09507} & \cellcolor[gray]{.8}\num{0.104719} & \num{0.098898} & \num{0.161702} & \num{0.12766} & \num{0.161702} \\
            iva\_kibo\_tag & \cellcolor[gray]{.8}\num{0.443206} & \num{0.305245} & \num{0.425435} & \num{0.134868} & \num{0.036184} & \num{0.134868} \\
            \bottomrule
        \end{tabular}
    }
\end{table*}
